Game-Theoretic Robust Reinforcement Learning Handles Temporally-Coupled Perturbations

Deploying reinforcement learning (RL) systems requires robustness to uncertainty and model misspecification, yet prior robust RL methods typically only study noise introduced independently across time. However, practical sources of uncertainty are usually coupled across time. We formally introduce temporally-coupled perturbations, presenting a novel challenge for existing robust RL methods. To tackle this challenge, we propose GRAD, a novel game-theoretic approach that treats the temporally-coupled robust RL problem as a partially observable two-player zero-sum game. By finding an approximate equilibrium within this game, GRAD optimizes for general robustness against temporally-coupled perturbations. Experiments on continuous control tasks demonstrate that, compared with prior methods, our approach achieves a higher degree of robustness to various types of attacks on different attack domains, both in settings with temporally-coupled perturbations and decoupled perturbations.

==> algorithms/DO.tex <==
\begin{algorithm}[tb]
  \caption{Double Oracle \cite{double_oracle}}
  \label{double_oracle}
\begin{algorithmic}
 \STATE {\bfseries Result:} Nash Equilibrium
  \STATE {\bfseries Input:} Initial population $\Pi^0$
  \REPEAT[for $t=0,1,\ldots$]
  \STATE $\pi^r \gets$ NE in game restricted to strategies in $\Pi^t$
  \FOR{$i \in \{1,2\}$}
  \STATE Find a best response $\beta_i \gets \mathbb{BR}_i(\pi^r_{-i})$
  \STATE $\Pi^{t+1}_i \gets \Pi^t_i \cup \{\beta_i\}$
  \ENDFOR
  \UNTIL{No novel best response exists for either player}
  \STATE {\bfseries Return:} $\pi^r$
\end{algorithmic}
\end{algorithm}


==> algorithms/MB-GRAD.tex <==
\begin{figure}[t]
\vspace{-2em}
\begin{algorithm}[H]
\caption{\oursfull (\ours)}
\label{alg:ours}
\begin{algorithmic}
  \STATE \textbf{Input:} Initial policies for agent $\Pi_a$ and adversary $\Pi_v$
  \STATE Initialize model $M_a$ for the agent using ME-TRPO
  \STATE Initialize empty set for storing explored policies: $\Pi_a^{explored} = \emptyset, \Pi_v^{explored} = \emptyset$

  \STATE Compute initial expected utilities: $U^{\Pi}$ for each joint policy $(\pi_a, \pi_v) \in \Pi$

  \STATE Compute initial meta-Nash equilibrium: $\sigma_a, \sigma_v$ based on $U^{\Pi}$

  \FOR {epoch in $\{1, 2, \ldots\}$ }
    \FOR {$i$ in $\{1, 2, \ldots, N_{\pi_a}\}$ }
      \STATE Sample adversary policy: $\pi_v \sim \sigma_v$
      \STATE Generate trajectories: $\mathcal{D}_{\pi_a'} = \{(\hat{s}_t^k, a_t^k, r_t^k, \hat{s}_{t+1}^k)\}_{k=1}^B$ against $\pi_v$ using $M_a$ (if fixed adversary only attacks action space, $\hat{s}_t = s_t$)
      \STATE Train agent policy $\pi_a'$ with $\mathcal{D}_{\pi_a'}$ using ME-TRPO (update $M_a$)
      \STATE $\Pi_a^{explored} = \Pi_a^{explored} \cup \{\pi_a'\}$
    \ENDFOR

    \FOR {$i$ in $\{1, 2, \ldots, N_{\pi_v}\}$ }
      \STATE Sample agent policy: $\pi_a \sim \sigma_a$
      \STATE Generate trajectories: $\mathcal{D}_{\pi_v'} = \{(s_t^k, \bar{a}_t^k, -r_t^k, s_{t+1}^k)\}_{k=1}^B$ with actual states $s_t$ and actions $\bar{a}_t$ taken by $\pi_a$
      \STATE Add perturbations to $\hat{s}_t^k$ in $\mathcal{D}_{\pi_v'}$ based on $\bar{a}_t$ (adversary's attack on agent's model)
      \STATE Train adversary policy $\pi_v'$ with the perturbed $\mathcal{D}_{\pi_v'}$
      \STATE $\Pi_v^{explored} = \Pi_v^{explored} \cup \{\pi_v'\}$
    \ENDFOR

    \STATE Update $U^{\Pi}$ based on newly explored policies $(\Pi_a^{explored}, \Pi_v^{explored})$
    \STATE Re-compute meta-strategies: $\sigma_a, \sigma_v$ based on the updated $U^{\Pi}$
  \ENDFOR

  \STATE \textbf{Return:} Current meta-Nash equilibrium on whole population: $\sigma_a, \sigma_v$
\end{algorithmic}
\end{algorithm}
\vspace{-2em}
\end{figure}


==> algorithms/PSRO.tex <==
\begin{algorithm}[tb]
  \caption{Pipeline Policy-Space Response Oracles (P2SRO) \cite{mcaleer2020pipeline}}
  \label{p2sro}
\begin{algorithmic}
  \STATE \textbf{Input:} Initial policy sets for all players $\Pi^f$
  \STATE Compute expected utilities as empirical payoff matrix $U^{\Pi}$ for each joint $\pi \in \Pi^f$
  \STATE Compute meta-Nash equilibrium $\sigma^{*,j}$ over fixed policies ($\Pi^f$)
  \FOR {epoch in $\{1,2,\ldots\}$}
  \FOR{\textbf{all} $\pi^{j}\in\Pi^a$ (active policies) in parallel}
  \FOR {player $i\in \{1,2\}$} 
  \STATE Sample $\pi_{-i}\sim\sigma_{-i}^{*,j}$
  \STATE Train $\pi_i^j$ against $\pi_{-i}$
  \ENDFOR
  \IF{$\pi^j$ plateaus and $\pi^j$ is the lowest active policy}
  \STATE $\Pi^{f}=\Pi^f\cup\{\pi^j\}$
  \STATE Initialize new active policy at a higher level than all existing active policies
  \STATE Compute missing entries in $U^{\Pi}$ from $\Pi$
  \STATE Compute meta Nash equilibrium for each active policy
  \ENDIF
  \ENDFOR
  \STATE Periodically compute meta Nash equilibrium for each active policy
  \ENDFOR
  \STATE \textbf{Return:} current meta Nash equilibrium on whole population $\sigma^{*}$
\end{algorithmic}
\end{algorithm}
\vspace{-0.5em}

==> figures/action.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{color0}{HTML}{E0D5BE}
\definecolor{color1}{HTML}{d0b3c2}
\definecolor{color2}{HTML}{b1c2a3}
\definecolor{color3}{HTML}{C7495C}
\definecolor{color4}{HTML}{c9d1de}

\begin{axis}[
height=3cm,
width=\textwidth,
scale only axis,
axis line style={white!15!black},
legend cell align={left},
legend columns = {2, 3},
legend style={
  fill opacity=0,
  draw opacity=1,
  text opacity=1,
  at={(0.53,1.01)},
  anchor=north,
  draw=none,
  font=\scriptsize
},
xtick pos = lower,
tick align=outside,
x grid style={white!80!black},
xmin=-0.7, xmax=5,
xtick style={color=white!15!black},
xtick={0.55,2.3,3.9},
xticklabels={\fontsize{5}{0}\selectfont{No Attack}, \fontsize{5}{0}\selectfont{Standard}, \fontsize{5}{0}\selectfont{Temporally-coupled}},
xtick style={color=white!15!black, font=\scriptsize},
xlabel={\fontsize{7}{0}\selectfont{Action Attacks}},
y grid style={white!80!black},
ylabel={\fontsize{7}{0}\selectfont{Average normalized rewards}},
ymin=-0.1, ymax=1.6,
ytick style={color=white!15!black, font=\fontsize{4pt}{0}\selectfont},
y grid style={white},
tick label style={font=\fontsize{4pt}{0}\selectfont},
ymajorgrids,
]

\draw[draw=white!93.3333333333333!black,fill=color4,very thin,postaction={pattern=grid, pattern color=white!90!black}] (axis cs:-0.2,0) rectangle (axis cs:0.1,0.249);
\draw[draw=white!93.3333333333333!black,fill=color0,very thin,postaction={pattern=crosshatch, pattern color=white!90!black}] (axis cs:0.1,0) rectangle (axis cs:0.4,0.68);
\draw[draw=white!93.3333333333333!black,fill=color1,very thin,postaction={pattern=north west lines, pattern color=white!90!black}] (axis cs:0.4,0) rectangle (axis cs:0.7,0.611);
\draw[draw=white!93.3333333333333!black,fill=color2,very thin,postaction={pattern=north east lines, pattern color=white!90!black}] (axis cs:0.7,0) rectangle (axis cs:1.0,0.644);
\draw[draw=white!93.3333333333333!black,fill=color3,very thin,postaction={pattern color=white!90!black}] (axis cs:1.0,0) rectangle (axis cs:1.3,0.643);

\draw[draw=white!93.3333333333333!black,fill=color4,very thin,postaction={pattern=grid, pattern color=white!90!black}] (axis cs:1.7,0) rectangle (axis cs:2.0,0.091);
\draw[draw=white!93.3333333333333!black,fill=color0,very thin,postaction={pattern=crosshatch, pattern color=white!90!black}] (axis cs:2.0,0) rectangle (axis cs:2.3,0.752);
\draw[draw=white!93.3333333333333!black,fill=color2,very thin,postaction={pattern=north east lines, pattern color=white!90!black}] (axis cs:2.3,0) rectangle (axis cs:2.6,0.819);
\draw[draw=white!93.3333333333333!black,fill=color3,very thin,postaction={pattern color=white!90!black}] (axis cs:2.6,0) rectangle (axis cs:2.9,0.894);

\draw[draw=white!93.3333333333333!black,fill=color4,very thin,postaction={pattern=grid, pattern color=white!90!black}] (axis cs:3.3,0) rectangle (axis cs:3.6,0.072);
\draw[draw=white!93.3333333333333!black,fill=color1,very thin,postaction={pattern=north west lines, pattern color=white!90!black}] (axis cs:3.6,0) rectangle (axis cs:3.9,0.748);
\draw[draw=white!93.3333333333333!black,fill=color2,very thin,postaction={pattern=north east lines, pattern color=white!90!black}] (axis cs:3.9,0) rectangle (axis cs:4.2,0.765);
\draw[draw=white!93.3333333333333!black,fill=color3,very thin,postaction={pattern color=white!90!black}] (axis cs:4.2,0) rectangle (axis cs:4.5,0.913);

\addlegendimage{ybar,ybar legend,draw=white!93.3333333333333!black,fill=color4,opacity=0.8,very thin,postaction={pattern=grid, pattern color=white!90!black, fill opacity=0.8}}
\addlegendentry{\tiny{AR-PPO}}
\addlegendimage{ybar,ybar legend,draw=white!93.3333333333333!black,fill=color0,opacity=0.8,very thin,postaction={pattern=crosshatch, pattern color=white!90!black, fill opacity=0.8}}
\addlegendentry{\tiny{AC-ATLA-PPO}}
\addlegendimage{ybar,ybar legend,draw=white!93.3333333333333!black,fill=color1,opacity=0.8,very thin,postaction={pattern=north west lines, pattern color=white!90!black, fill opacity=0.8}}
\addlegendentry{\tiny{AC-ATLA-PPO*}}
\addlegendimage{ybar,ybar legend,draw=white!93.3333333333333!black,fill=color2,opacity=0.8,very thin,postaction={pattern=north east lines, pattern color=white!90!black, fill opacity=0.8}}
\addlegendentry{\tiny{WocaR-PPO}}
\addlegendimage{ybar,ybar legend,draw=white!93.3333333333333!black,fill=color3,opacity=0.8,very thin,postaction={, pattern color=white!90!black, fill opacity=0.8}}
\addlegendentry{\tiny{\textbf{\ours(Ours)}}}
%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:0,0.766)
%--(axis cs:0,0.113);

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:1.65,1)
%--(axis cs:1.65,0);

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%%0 0.766
%1.65 0
%};

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0 0.113
%1.65 1
%};

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:0.3,0.864)
%--(axis cs:0.3,0.01);

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:3,0)
%--(axis cs:3,1);

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0.3 0.864
%3 1
%};

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0.3 0.01
%3 2806
%};

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:0.6,0.848)
%--(axis cs:0.6,0.173);

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:1.95,2715)
%--(axis cs:1.95,3147);

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:3.3,2468)
%--(axis cs:3.3,2942);

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0.6 0.848
%1.95 2715
%3.3 2468
%};
%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0.6 0.173
%1.95 3147
%3.3 2942
%};

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:0.9,0.721)
%--(axis cs:0.9,0.069);

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:2.25,3055)
%--(axis cs:2.25,3539);

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:3.6,3082)
%--(axis cs:3.6,3824);

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0.9 0.721
%2.25 3055
%3.6 3082
%};

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0.9 0.069
%2.25 3539
%3.6 3824
%};

\end{axis}

\end{tikzpicture}


==> figures/adaptive.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{color0}{HTML}{E0D5BE}
\definecolor{color1}{HTML}{d0b3c2}
\definecolor{color2}{HTML}{b1c2a3}
\definecolor{color3}{HTML}{C7495C}

\begin{axis}[
height=3cm,
width=\textwidth,
scale only axis,
axis line style={white!15!black},
legend cell align={left},
legend columns=2,
legend style={
  fill opacity=0,
  draw opacity=1,
  text opacity=1,
  at={(0.53,1.01)},
  anchor=north,
  draw=none,
  font=\scriptsize
},
xtick pos = lower,
tick align=outside,
x grid style={white!80!black},
xmin=-0.7, xmax=4.3,
xtick style={color=white!15!black},
xtick={0.45,1.95,3.3},
xticklabels={\fontsize{5}{0}\selectfont{No Attack}, \fontsize{5}{0}\selectfont{Standard}, \fontsize{5}{0}\selectfont{Temporally-coupled}},
xtick style={color=white!15!black, font=\scriptsize},
xlabel={\fontsize{7}{0}\selectfont{State or Action Attacks}},
y grid style={white!80!black},
ylabel={\fontsize{7}{0}\selectfont{Average normalized rewards}},
ymin=-0.1, ymax=1.3,
ytick style={color=white!15!black, font=\fontsize{4pt}{0}\selectfont},
y grid style={white},
tick label style={font=\fontsize{4pt}{0}\selectfont},
ymajorgrids,
]

\draw[draw=white!93.3333333333333!black,fill=color0,very thin,postaction={pattern=crosshatch, pattern color=white!90!black}] (axis cs:-0.15,0) rectangle (axis cs:0.15,0.527);
\addlegendimage{ybar,ybar legend,draw=white!93.3333333333333!black,fill=color0,opacity=0.8,very thin,postaction={pattern=crosshatch, pattern color=white!90!black, fill opacity=0.8}}
\addlegendentry{\tiny{SA-ATLA-PPO}}

\draw[draw=white!93.3333333333333!black,fill=color0,very thin,postaction={pattern=crosshatch, pattern color=white!90!black}] (axis cs:1.50,0) rectangle (axis cs:1.80,0.282);
\draw[draw=white!93.3333333333333!black,fill=color1,very thin,postaction={pattern=north west lines, pattern color=white!90!black}] (axis cs:0.15,0) rectangle (axis cs:0.45,0.507);
\addlegendimage{ybar,ybar legend,draw=white!93.3333333333333!black,fill=color1,opacity=0.8,very thin,postaction={pattern=north west lines, pattern color=white!90!black, fill opacity=0.8}}
\addlegendentry{\tiny{SA-ATLA-PPO*}}

\draw[draw=white!93.3333333333333!black,fill=color1,very thin,postaction={pattern=north west lines, pattern color=white!90!black}] (axis cs:2.85,0) rectangle (axis cs:3.15,0.273);
\draw[draw=white!93.3333333333333!black,fill=color2,opacity=0.8,very thin,postaction={pattern=north east lines, pattern color=white!90!black, fill opacity=0.8}] (axis cs:0.45,0) rectangle (axis cs:0.75,0.525);
\addlegendimage{ybar,ybar legend,draw=white!93.3333333333333!black,fill=color2,opacity=0.8,very thin,postaction={pattern=north east lines, pattern color=white!90!black, fill opacity=0.8}}
\addlegendentry{\tiny{WocaR-PPO}}

\draw[draw=white!93.3333333333333!black,fill=color2,opacity=0.8,very thin,postaction={pattern=north east lines, pattern color=white!90!black, fill opacity=0.8}] (axis cs:1.80,0) rectangle (axis cs:2.10,0.416);
\draw[draw=white!93.3333333333333!black,fill=color2,opacity=0.8,very thin,postaction={pattern=north east lines, pattern color=white!90!black, fill opacity=0.8}] (axis cs:3.15,0) rectangle (axis cs:3.45,0.335);
\draw[draw=white!93.3333333333333!black,fill=color3,very thin] (axis cs:0.75,0) rectangle (axis cs:1.05,0.517);
\addlegendimage{ybar,ybar legend,draw=white!93.3333333333333!black,fill=color3,opacity=0.8,very thin,postaction={fill opacity=0.8}}
\addlegendentry{\tiny{\textbf{\ours(Ours)}}}

\draw[draw=white!93.3333333333333!black,fill=color3,very thin] (axis cs:2.10,0) rectangle (axis cs:2.40,0.731);
\draw[draw=white!93.3333333333333!black,fill=color3,very thin] (axis cs:3.45,0) rectangle (axis cs:3.75,0.764);
%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:0,0.766)
%--(axis cs:0,0.113);

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:1.65,1)
%--(axis cs:1.65,0);

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%%0 0.766
%1.65 0
%};

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0 0.113
%1.65 1
%};

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:0.3,0.864)
%--(axis cs:0.3,0.01);

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:3,0)
%--(axis cs:3,1);

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0.3 0.864
%3 1
%};

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0.3 0.01
%3 2806
%};

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:0.6,0.848)
%--(axis cs:0.6,0.173);

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:1.95,2715)
%--(axis cs:1.95,3147);

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:3.3,2468)
%--(axis cs:3.3,2942);

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0.6 0.848
%1.95 2715
%3.3 2468
%};
%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0.6 0.173
%1.95 3147
%3.3 2942
%};

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:0.9,0.721)
%--(axis cs:0.9,0.069);

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:2.25,3055)
%--(axis cs:2.25,3539);

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:3.6,3082)
%--(axis cs:3.6,3824);

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0.9 0.721
%2.25 3055
%3.6 3082
%};

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0.9 0.069
%2.25 3539
%3.6 3824
%};

\end{axis}

\end{tikzpicture}


==> figures/eps_.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}[scale=0.5]

\definecolor{color0}{rgb}{0.917647058823529,0.917647058823529,0.949019607843137}
\definecolor{color1}{rgb}{0.372549019607843,0.619607843137255,0.627450980392157}
\definecolor{color2}{rgb}{0.133333333333333,0.545098039215686,0.133333333333333}
\definecolor{color3}{rgb}{0.576470588235294,0.43921568627451,0.858823529411765}
%\definecolor{color4}{rgb}{0.392156862745098,0.584313725490196,0.929411764705882}
%\definecolor{color5}{rgb}{0.862745098039216,0.0784313725490196,0.235294117647059}
\definecolor{color4}{HTML}{b1c2a3}
\definecolor{color5}{HTML}{C7495C}

\begin{axis}[
axis background/.style={fill=white},
axis line style={black},
legend cell align={left},
legend style={
  fill opacity=0.2,
  draw opacity=1,
  text opacity=1,
  at={(0.5,0.9)},
  anchor=north west,
  draw=none,
  fill=color0
},
tick align=outside,
x grid style={color=white},
xlabel={Temporally-coupled constraint $\bar{\epsilon}$},
xmajorgrids=false,
% xmajorticks=false,
xmin=-0.005, xmax=0.11,
xtick style={color=white!15!black},
xtick={ 0.01, 0.02, 0.05, 0.1},
xticklabels={ \num{0.01}, \num{0.02}, \num{0.05}, \num{0.1}},
y grid style={color=white},
ylabel={Average rewards under attacks},
ymajorgrids=false,
% ymajorticks=false,
ymin=1500, ymax=6000,
ytick style={color=white!15!black}
]
\addplot [line width=0.8pt, color4, color4, mark=pentagon*, mark size=3.2, mark options={solid}]
table{%
x  y
0  5638
0.01 3045
0.015 2356
0.02 1974
0.05 2030
0.1 2214
};
\addlegendentry{WocaR-PPO}
\addplot [line width=0.8pt, color5, mark=*, mark size=2.9, mark options={solid}]
table{%
x  y
0 5603
0.01 3561
0.015 3076
0.02 2864
0.05 2894
0.1 2814
};
\addlegendentry{\textbf{\ours(Ours)}}
\end{axis}
\end{tikzpicture}


==> figures/exp.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[!t]{0.32\textwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{figures/state}}
        \vspace{-1em}
        \label{sfig:state}
    \end{subfigure}
    \begin{subfigure}[!t]{0.32\textwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{figures/action}}
        \vspace{-1em}
        \label{sfig:action}
    \end{subfigure}
    \begin{subfigure}[!t]{0.32\textwidth}
        \centering
        \resizebox{\textwidth}{!}{\input{figures/adaptive}}
        \vspace{-1em}
        \label{sfig:adaptable}
    \end{subfigure}
\caption{Histograms of normalized average rewards for \ours and baselines across five environments, which mitigate the impact of varying reward ranges across
environments. Each bar represents the distribution of rewards obtained by robust agents, as presented in Tables~\ref{tab:table_state}, \ref{tab:table_action}, and \ref{tab:table_adaptable}. }
\label{fig:exp}
\vspace{-1em}
\end{figure}

==> figures/state.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{color0}{HTML}{E0D5BE}
\definecolor{color1}{HTML}{d0b3c2}
\definecolor{color2}{HTML}{b1c2a3}
\definecolor{color3}{HTML}{C7495C}

\begin{axis}[
height=3cm,
width=\textwidth,
scale only axis,
axis line style={white!15!black},
legend cell align={left},
legend columns=2,
legend style={
  fill opacity=0,
  draw opacity=1,
  text opacity=1,
  at={(0.53,1.01)},
  anchor=north,
  draw=none,
  font=\scriptsize
},
xtick pos = lower,
tick align=outside,
x grid style={white!80!black},
xmin=-0.7, xmax=4.3,
xtick style={color=white!15!black},
xtick={0.45,1.95,3.3},
xticklabels={\fontsize{5}{0}\selectfont{No Attack}, \fontsize{5}{0}\selectfont{Standard}, \fontsize{5}{0}\selectfont{Temporally-coupled}},
xtick style={color=white!15!black, font=\scriptsize},
xlabel={\fontsize{7}{0}\selectfont{State Attacks}},
y grid style={white!80!black},
ylabel={\fontsize{7}{0}\selectfont{Average normalized rewards}},
ymin=-0.1, ymax=1.3,
ytick style={color=white!15!black, font=\fontsize{4pt}{0}\selectfont},
y grid style={white},
tick label style={font=\fontsize{4pt}{0}\selectfont},
ymajorgrids,
]

\draw[draw=white!93.3333333333333!black,fill=color0,very thin,postaction={pattern=crosshatch, pattern color=white!90!black}] (axis cs:-0.15,0) rectangle (axis cs:0.15,0.44);
\addlegendimage{ybar,ybar legend,draw=white!93.3333333333333!black,fill=color0,opacity=0.8,very thin,postaction={pattern=crosshatch, pattern color=white!90!black, fill opacity=0.8}}
\addlegendentry{\tiny{PA-ATLA-PPO}}

\draw[draw=white!93.3333333333333!black,fill=color0,very thin,postaction={pattern=crosshatch, pattern color=white!90!black}] (axis cs:1.50,0) rectangle (axis cs:1.80,0.198);
\draw[draw=white!93.3333333333333!black,fill=color1,very thin,postaction={pattern=north west lines, pattern color=white!90!black}] (axis cs:0.15,0) rectangle (axis cs:0.45,0.437);
\addlegendimage{ybar,ybar legend,draw=white!93.3333333333333!black,fill=color1,opacity=0.8,very thin,postaction={pattern=north west lines, pattern color=white!90!black, fill opacity=0.8}}
\addlegendentry{\tiny{PA-ATLA-PPO*}}

\draw[draw=white!93.3333333333333!black,fill=color1,very thin,postaction={pattern=north west lines, pattern color=white!90!black}] (axis cs:2.85,0) rectangle (axis cs:3.15,0.19);
\draw[draw=white!93.3333333333333!black,fill=color2,opacity=0.8,very thin,postaction={pattern=north east lines, pattern color=white!90!black, fill opacity=0.8}] (axis cs:0.45,0) rectangle (axis cs:0.75,0.511);
\addlegendimage{ybar,ybar legend,draw=white!93.3333333333333!black,fill=color2,opacity=0.8,very thin,postaction={pattern=north east lines, pattern color=white!90!black, fill opacity=0.8}}
\addlegendentry{\tiny{WocaR-PPO}}

\draw[draw=white!93.3333333333333!black,fill=color2,opacity=0.8,very thin,postaction={pattern=north east lines, pattern color=white!90!black, fill opacity=0.8}] (axis cs:1.80,0) rectangle (axis cs:2.10,0.491);
\draw[draw=white!93.3333333333333!black,fill=color2,opacity=0.8,very thin,postaction={pattern=north east lines, pattern color=white!90!black, fill opacity=0.8}] (axis cs:3.15,0) rectangle (axis cs:3.45,0.446);
\draw[draw=white!93.3333333333333!black,fill=color3,very thin] (axis cs:0.75,0) rectangle (axis cs:1.05,0.395);
\addlegendimage{ybar,ybar legend,draw=white!93.3333333333333!black,fill=color3,opacity=0.8,very thin,postaction={fill opacity=0.8}}
\addlegendentry{\tiny{\textbf{\ours(Ours)}}}

\draw[draw=white!93.3333333333333!black,fill=color3,very thin] (axis cs:2.10,0) rectangle (axis cs:2.40,0.781);
\draw[draw=white!93.3333333333333!black,fill=color3,very thin] (axis cs:3.45,0) rectangle (axis cs:3.75,0.8);
%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:0,0.766)
%--(axis cs:0,0.113);

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:1.65,1)
%--(axis cs:1.65,0);

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%%0 0.766
%1.65 0
%};

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0 0.113
%1.65 1
%};

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:0.3,0.864)
%--(axis cs:0.3,0.01);

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:3,0)
%--(axis cs:3,1);

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0.3 0.864
%3 1
%};

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0.3 0.01
%3 2806
%};

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:0.6,0.848)
%--(axis cs:0.6,0.173);

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:1.95,2715)
%--(axis cs:1.95,3147);

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:3.3,2468)
%--(axis cs:3.3,2942);

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0.6 0.848
%1.95 2715
%3.3 2468
%};
%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0.6 0.173
%1.95 3147
%3.3 2942
%};

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:0.9,0.721)
%--(axis cs:0.9,0.069);

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:2.25,3055)
%--(axis cs:2.25,3539);

%\path [draw=white!41.1764705882353!black, line width=0.48pt]
%(axis cs:3.6,3082)
%--(axis cs:3.6,3824);

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0.9 0.721
%2.25 3055
%3.6 3082
%};

%\addplot [line width=0.48pt, white!41.1764705882353!black, opacity=1, mark=-, mark size=1.3, mark options={solid}, only marks]
%table {%
%0.9 0.069
%2.25 3539
%3.6 3824
%};

\end{axis}

\end{tikzpicture}


==> math_commands.tex <==

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> packages.tex <==
\usepackage{iclr2024_conference,times}

\usepackage{pdfpages}
\usepackage{amsmath}
\usepackage{amsfonts}
% \usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{multirow}
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{algorithm}
\usepackage{algorithmic}


\usepackage[backref=page,colorlinks=true,linkcolor=blue,citecolor=green,urlcolor=blue]{hyperref}
\usepackage{url}
\usepackage{graphicx}
\usepackage{bbm}
\usepackage{placeins}
\usepackage{adjustbox}
\usepackage{xcolor}
\usepackage{scalerel}
\setlength\parindent{0pt}

\usepackage{natbib}
\usepackage[outdir=./]{epstopdf}
\usepackage{graphicx,float,pgfplots,wrapfig,sidecap,lipsum}

\usepackage{colortbl}
\usepackage{diagbox} 
\usepackage{tablefootnote}
\usepackage[font=small,labelfont=bf]{caption}
\usepackage{subcaption}
\usepackage{subfloat}

\usepackage{tikz}
\usetikzlibrary{fit}
\usetikzlibrary{calc,shapes}
\usetikzlibrary{decorations.pathmorphing} % noisy shapes
\usetikzlibrary{fit}					% fitting shapes to coordinates
\usetikzlibrary{backgrounds}	
\usetikzlibrary{pgfplots.groupplots}
\usepackage{siunitx}

\usepackage[utf8]{inputenc}
\usepackage{pgfplots}
\usepgfplotslibrary{groupplots,dateplot}
\usetikzlibrary{patterns,shapes.arrows}
\pgfplotsset{compat=newest}

\usepackage{xspace}
\usepackage{soul}
\usepackage{booktabs}
\usepackage{bm}

\usepackage{listings}

\usepackage{enumitem}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}

\lstset{style=mystyle}

==> tables/table_action.tex <==
\begin{table*}[!t]
\vspace{-0.5em}
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{4pt}
% \setlength{\arrayrulewidth}{1pt}
\begin{tabular}{p{2.5cm}<{\centering} | p{2.7cm}<{\centering}| p{2.5cm}<{\centering}| p{2.5cm}<{\centering}|p{2.5cm}<{\centering}| p{2.5cm}<{\centering}|p{2.5cm}<{\centering}}
\toprule
\multicolumn{2}{c|}{\textbf{Environment}}     & \textbf{Hopper}         & \textbf{Walker2d}  & \textbf{Halfcheetah} & \textbf{Ant} & \textbf{Humanoid} \\
\midrule
\multicolumn{2}{c|}{$\epsilon$ / action dim}     & 0.2 / 3      & 0.2 / 6 & 0.2 / 6 & 0.15 / 8 & 0.15 / 17 \\
\midrule
\multirow{4}{5em}{\begin{tabular}[c]{@{}c@{}}{\textbf{Natural}}\\\textbf{Reward}\\\textbf{(no attack)}\end{tabular}} & AC-ATLA-PPO & 3576 $\pm$ 43  & 4228 $\pm$ 26  & 5915 $\pm$ 28  & 5557 $\pm$ 33 & 6014 $\pm$ 49 \\
&  AC-ATLA-PPO* & 3492 $\pm$ 28 & 4052 $\pm$ 29 & 5853 $\pm$ 32 & 5549 $\pm$ 21 & 5980 $\pm$ 30 \\
&  AR-PPO & 3188 $\pm$ 28 & 3767 $\pm$ 15 &  5248 $\pm$ 35  & 5074 $\pm$ 34  & 5379 $\pm$ 42  \\
&  \textbf{\ours (Ours)} & 3482 $\pm$ 20 & 4159 $\pm$ 26 & 6047 $\pm$ 29 & 5512 $\pm$ 38 & 5894 $\pm$ 35 \\
\midrule
\multirow{4}{5em}{\begin{tabular}[c]{@{}c@{}}{\textbf{Best}}\\\textbf{Standard}\\\textbf{Action Attack}\end{tabular}} 
& AC-ATLA-PPO &  2872  $\pm$ 18  & 3108 $\pm$ 22  & 3994 $\pm$ 41 & 2752 $\pm$ 33 & 3120 $\pm$ 39 \\
&  AR-PPO &  1235 $\pm$ 26 & 1305 $\pm$ 31 & 1523 $\pm$ 24  & 1120 $\pm$ 10  & 1117 $\pm$ 37  \\
&  WocaR-PPO & 2943 $\pm$ 18 & 3269 $\pm$ 28 & 3840 $\pm$ 29 & 3345 $\pm$ 21 & 3419 $\pm$ 37 \\
&  \cellcolor{lightgray}{\textbf{\ours (Ours)}} & \cellcolor{lightgray}{\textbf{3039 $\pm$ 20}} & \cellcolor{lightgray}{\textbf{3298 $\pm$ 35} }& \cellcolor{lightgray}{\textbf{4016 $\pm$ 28}} & \cellcolor{lightgray}{\textbf{3569 $\pm$ 26}} & \cellcolor{lightgray}{\textbf{4106 $\pm$ 32}} \\
\midrule
\multirow{3}{5em}{\begin{tabular}[c]{@{}c@{}}{\textbf{Best}}\\\textbf{Temporally-}\\\textbf{Coupled}\\\textbf{Action Attack}\end{tabular}} & AC-ATLA-PPO* & 2625 $\pm$ 15 & 2780 $\pm$ 26 & 3815 $\pm$ 36 & 3382 $\pm$ 27 & 3092 $\pm$ 17 \\
&  AR-PPO &  974 $\pm$ 15 & 1120 $\pm$ 28 & 1439 $\pm$ 21  & 679 $\pm$ 18  & 585 $\pm$ 29   \\
&  WocaR-PPO & 2673 $\pm$ 28 & 2860 $\pm$ 32 & 4018 $\pm$ 37 & 3260 $\pm$ 27 & 3132 $\pm$ 35 \\
&  \cellcolor{lightgray}{\textbf{\ours (Ours)}} & \cellcolor{lightgray}{\textbf{3125 $\pm$ 26}} & \cellcolor{lightgray}{\textbf{3179 $\pm$ 20} }& \cellcolor{lightgray}{\textbf{4320 $\pm$ 27}} & \cellcolor{lightgray}{\textbf{3619 $\pm$ 34}} & \cellcolor{lightgray}{\textbf{4156 $\pm$ 29}} \\
\bottomrule
\end{tabular}}
% \vspace{-1em}
\caption{Average episode rewards $\pm$ standard error for over 100 episodes action robust baselines and our \textbf{\ours} under no attack and best action attacks. }
\label{tab:table_action}
\vspace{-1.5em}
\end{table*}

==> tables/table_adaptable.tex <==
\begin{table*}[!t]
\vspace{-0.5em}
\centering
\renewcommand{\arraystretch}{1.3}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{4pt}
% \setlength{\arrayrulewidth}{1pt}
\begin{tabular}{p{2.5cm}<{\centering} | p{2.7cm}<{\centering}| p{2.5cm}<{\centering}| p{2.5cm}<{\centering}|p{2.5cm}<{\centering}| p{2.5cm}<{\centering}|p{2.5cm}<{\centering}}
\toprule
\multicolumn{2}{c|}{\textbf{Environment}}     & \textbf{Hopper}         & \textbf{Walker2d}  & \textbf{Halfcheetah} & \textbf{Ant} & \textbf{Humanoid} \\
\midrule
\multirow{3}{5em}{\begin{tabular}[c]{@{}c@{}}{\textbf{Natural}}\\\textbf{Reward}\\\textbf{(no attack)}\end{tabular}} & SA-ATLA-PPO & 3498 $\pm$ 34  & 4195 $\pm$ 36  &  6078 $\pm$ 38  & 5442 $\pm$ 28 & 5913 $\pm$ 34 \\
&  SA-ATLA-PPO* & 3372 $\pm$ 29 & 4219 $\pm$ 31 & 5979 $\pm$ 37 & 5510 $\pm$ 29 & 5949 $\pm$ 22\\
&  \textbf{\ours (Ours)} & 3420 $\pm$ 18 & 4218 $\pm$ 27 & 6123 $\pm$ 18 & 5517 $\pm$ 21 & 5799 $\pm$ 27 \\
\midrule
\multirow{3}{5em}{\begin{tabular}[c]{@{}c@{}}{\textbf{Best}}\\\textbf{Standard}\\\textbf{SA Attack}\end{tabular}} 
& SA-ATLA-PPO & 2294 $\pm$ 27 & 2503 $\pm$ 34 & 4028 $\pm$ 28 & 2750 $\pm$ 32 & 1981 $\pm$ 25 \\
&  WocaR-PPO & 2469 $\pm$ 18 &  2594 $\pm$ 32 &  4012 $\pm$ 26 & 3024 $\pm$ 23  & 2263 $\pm$ 28  \\
&  \cellcolor{lightgray}{\textbf{\ours (Ours)}} & \cellcolor{lightgray}{\textbf{2846 $\pm$ 24}} & \cellcolor{lightgray}{\textbf{2897 $\pm$ 31} }& \cellcolor{lightgray}{\textbf{4168 $\pm$ 37}} & \cellcolor{lightgray}{\textbf{3286 $\pm$ 20}} & \cellcolor{lightgray}{\textbf{3042 $\pm$ 24}} \\
\midrule
\multirow{3}{5em}{\begin{tabular}[c]{@{}c@{}}{\textbf{Best}}\\\textbf{\scriptsize{Temporally-coupled}}\\\textbf{SA Attack}\end{tabular}} & SA-ATLA-PPO* &1994 $\pm$ 20 & 2492 $\pm$ 28 & 3694 $\pm$ 23 & 3145 $\pm$ 26 & 1972 $\pm$ 19  \\
&  WocaR-PPO & 2297 $\pm$ 25 & 2497 $\pm$ 22 & 3935 $\pm$ 29 & 2887 $\pm$ 32 & 2180 $\pm$ 23 \\
&  \cellcolor{lightgray}{\textbf{\ours (Ours)}} & \cellcolor{lightgray}{\textbf{3051 $\pm$ 33}} & \cellcolor{lightgray}{\textbf{2932 $\pm$ 24} }& \cellcolor{lightgray}{\textbf{4096 $\pm$ 28}} & \cellcolor{lightgray}{\textbf{3336 $\pm$ 22}} & \cellcolor{lightgray}{\textbf{3295 $\pm$ 34}} \\
\bottomrule
\end{tabular}}
% \vspace{-1em}
\caption{Average episode rewards $\pm$ standard error over 100 episodes for adaptable adversarial defense baselines and our \textbf{\ours}.}
\label{tab:table_adaptable}
\vspace{-0.5em}
\end{table*}

==> tables/table_state.tex <==
\begin{table*}[!t]
\vspace{-0.5em}
\centering
\renewcommand{\arraystretch}{1.24}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{3pt}
% \setlength{\arrayrulewidth}{1pt}
\begin{tabular}{p{2.8cm}<{\centering} | p{2.5cm}<{\centering}| p{2.5cm}<{\centering}| p{2.5cm}<{\centering}|p{2.5cm}<{\centering}| p{2.5cm}<{\centering}|p{2.5cm}<{\centering}}
\toprule
\multicolumn{2}{c|}{\textbf{Environment}}     & \textbf{Hopper}         & \textbf{Walker2d}  & \textbf{Halfcheetah} & \textbf{Ant} & \textbf{Humanoid} \\
\midrule
\multicolumn{2}{c|}{$\epsilon$ / state dim }     & 0.075 / 11      & 0.05 / 17 & 0.15 / 17 & 0.15 / 111 & 0.1 / 376 \\
\midrule
\multirow{4}{5em}{\begin{tabular}[c]{@{}c@{}}{\textbf{Natural}}\\\textbf{Reward}\\\textbf{(no attack)}\end{tabular}} & PA-ATLA-PPO & 3425 $\pm$ 22 & 4153 $\pm$ 31 &  6175 $\pm$ 29 &  5340 $\pm$ 11 & 5792 $\pm$ 18 \\
&  PA-ATLA-PPO* & 3476 $\pm$ 31 & 4032 $\pm$ 29 & 6291 $\pm$ 37 & 5431 $\pm$ 28 & 5659 $\pm$ 19 \\
&  WocaR-PPO & 3588 $\pm$ 12 & 4102 $\pm$ 34 &  6032 $\pm$ 14 & 5576 $\pm$ 21 & 5781 $\pm$ 30 \\
&  \textbf{\ours (Ours)} & 3345 $\pm$ 15 & 4089 $\pm$ 24 & 6149 $\pm$ 27 & 5376 $\pm$ 21 & 5772 $\pm$ 23\\
\midrule
\multirow{3}{5em}{\begin{tabular}[c]{@{}c@{}}{\textbf{Best}}\\\textbf{Standard}\\\textbf{State Attack}\end{tabular}} 
& PA-ATLA-PPO & 2532 $\pm$ 31 & 2241 $\pm$ 17 & 3849 $\pm$ 28 & 2874 $\pm$ 25 & 1435 $\pm$ 22 \\
&  WocaR-PPO & 2570 $\pm$ 23 &  2715 $\pm$ 16 & 4225 $\pm$ 20 & 3145 $\pm$ 19 & 2236 $\pm$ 26 \\
&  \cellcolor{lightgray}{\textbf{\ours (Ours)}} & \cellcolor{lightgray}{\textbf{2899 $\pm$ 27}} & \cellcolor{lightgray}{\textbf{3108 $\pm$ 25} }& \cellcolor{lightgray}{\textbf{4447 $\pm$ 28}} & \cellcolor{lightgray}{\textbf{3397 $\pm$ 18}} & \cellcolor{lightgray}{\textbf{2787 $\pm$ 25}} \\
\midrule
\multirow{3}{5em}{\begin{tabular}[c]{@{}c@{}}{\textbf{Best}}\\\textbf{\scriptsize{Temporally-coupled}}\\\textbf{State Attack}\end{tabular}} & PA-ATLA-PPO* & 2286 $\pm$ 29  & 2095 $\pm$ 34 & 3572 $\pm$ 31 & 2594 $\pm$ 19 & 1462 $\pm$ 27 \\
&  WocaR-PPO & 2298 $\pm$ 13  & 2562 $\pm$ 18 & 4136 $\pm$ 28 & 3046 $\pm$ 10 & 1974 $\pm$ 33 \\
&  \cellcolor{lightgray}{\textbf{\ours (Ours)}} & \cellcolor{lightgray}{\textbf{2867 $\pm$ 36}} & \cellcolor{lightgray}{\textbf{2945 $\pm$ 27} }& \cellcolor{lightgray}{\textbf{4526 $\pm$ 29}} & \cellcolor{lightgray}{\textbf{3519 $\pm$ 24}} & \cellcolor{lightgray}{\textbf{2864 $\pm$ 28}} \\
\bottomrule
\end{tabular}}
% \vspace{-1em}
\caption{Average episode rewards $\pm$ standard error over 100 episodes for three state robust baselines and our \textbf{\ours}. \textbf{Bold} numbers indicate the best results under different types of attacks on state spaces. The \colorbox{lightgray}{gray} rows are the most robust agents.}
\label{tab:table_state}
\vspace{-1.5em}
\end{table*}

